Finding Patient Zero: Learning Contagion Source with Graph Neural Networks

Locating the source of an epidemic, or patient zero (P0), can provide critical insights into the infection's transmission course and allow efficient resource allocation. Existing methods use graph-theoretic centrality measures and expensive message-passing algorithms, requiring knowledge of the underlying dynamics and its parameters. In this paper, we revisit this problem using graph neural networks (GNNs) to learn P0. We establish a theoretical limit for the identification of P0 in a class of epidemic models. We evaluate our method against different epidemic models on both synthetic and a real-world contact network considering a disease with history and characteristics of COVID-19. % We observe that GNNs can identify P0 close to the theoretical bound on accuracy, without explicit input of dynamics or its parameters. In addition, GNN is over 100 times faster than classic methods for inference on arbitrary graph topologies. Our theoretical bound also shows that the epidemic is like a ticking clock, emphasizing the importance of early contact-tracing. We find a maximum time after which accurate recovery of the source becomes impossible, regardless of the algorithm used.

==> secs/bkup.tex <==

\section{Backup 2020-06-02}
% \begin{comment}
\subsection{Graph Isomorphism and Ambiguity of Patient Zero}
\begin{wrapfigure}{r}{0.6\textwidth}
% \includegraphics[width=.5\linewidth]{figs/hash-infected-subgraph138-BA-5-k_max200.pdf}
\includegraphics[width=.49\linewidth]{figs/hash-infected-subgraph100-RGG-200-k_max5.pdf}
\includegraphics[width=.49\linewidth]{figs/hash-infected-subgraph115-BA-200-k_max5.pdf}
\caption{Equivalence classes of the quick hashing method inspired by WL. 
Grey nodes are outside $G_I$. 
The colors indicate the equivalence classes. On the tree (right) $G_I$ has 115 nodes, but only $38$ distinguishable groups.
The Random Geometric Graph (left), however, with $|G_I|=100$ has $84$ groups. 
}
\label{fig:Ambiguity}
\vspace{-3mm}
\end{wrapfigure}
It may happen that the problem of finding P0 is unidentifiable 
when some nodes in the graph are identical. 
% \ry{separate the analyze of trees and general graphs}
For instance, when $G_I$ is a tree, if P0 is predicted to be a leaf, all leaves sharing the same parent are equally likely to be P0.
% \ry{this only happens if we have multiple patient zeros} \nd{no, even for a single P0, it's ambiguous.}. 
% If some nodes are truly indistinguishable, 
% our measure of accuracy should check P0 modulo an equivalence relations between nodes, i.e. automorphisms of the graph. 
In such cases, we need to assess the accuracy of our prediction modulo automorphisms $ \mathrm{Aut}({G}_I)$. %, requiring us to group equivalent nodes together. 
Finding $\mathrm{Aut}(G_I)$ is the Graph Isomorphism (GI) problem, which is in NP, but not known if it is NP-complete \cite{mckay1981practical}, with existing algorithm being at least exponential in $N$ \cite{MCKAY201494}.
% There exist many algorithms for GI \cite{MCKAY201494}, all of which are at least exponential in $N$. 
We choose to use a simpler heuristic inspired by the Weisfeiler-Lehman (WS) graph kernel \cite{weisfeiler1968reduction, shervashidze2011weisfeiler}. 
% The idea is to label the nodes by a sequence of numbers encoding the local structure of the graph around each node. 
A simple measure for encoding the local structure of the graph is the number nodes $n_i^{(l)}$ within a distance $l$ from node $i$. 
We label each node by the sequence $n_i =(n_i^{(1)},...,n^{(l_{\max})}_i) $.  
$n_i^{(1)}$ is the degree of node $i$ and we have $n_i^{(l)} = \theta(A_I^l) \mathbf{1}$
% \begin{equation}
%     n_i^l = \theta(A^l) \mathbf{1} \label{eq:nil}
% \end{equation}
with $A_I^l$ being the $l$th power of the adjacency matrix of the $G_I$ and $\theta(\cdot)$ the step function. % $\theta(x) = \{1, \mbox{ if} x>0; 0,\mbox{else}\} $ 


Figure \ref{fig:Ambiguity} shows that on trees there are many equivalent nodes, even non-leaf nodes.
However, the structure of contact networks where diseases spread is much more localized, similar to a %A good model for contact networks is a 
``Random Geometric Graph'' (RGG). 
Left of Figure \ref{fig:Ambiguity} shows that on RGG, the level of node equivalence is far less, with most nodes being distinguishable. 
In general, we find non-tree graphs with sufficient randomness (e.g. RGG and random graphs), there are very few equivalent nodes in small graphs. 
Hence, we believe in realistic settings this ambiguity won't play a major role in identifiability of P0.  
% \nd{but on tree BA we should definitely group nodes.}
% \end{comment}


\section{Backup 2020-05-31}
\subsection{Architecture}
Graph neural networks offer new promises for solving difficult inference problems on graphs. 
% The appealing factors of using graph neural networks for probabilistic inference compared to existing methods such as dynamic message passing is that they are ``model-free'' and do not reply on knowing the diffusion dynamics. 
%
We take the first step to compare the performance of graph neural networks for finding patient zeros versus the classic inference algorithms. Note that our goal in this work is not to propose a novel graph neural network architecture, but to understand the trade-off between different probabilistic inference methods in the context of contagion dynamics. 

\nd{Let's go over the detail of the architecture we use, make a diagram and rewrite this section. 
This could be moved to after theory, or appended to the section below. }
We employ a state-of-the-art graph neural network design, suggested by \cite{dwivedi2020benchmarking}. We make the following modifications to the model architecture to fit our problem.  
%
Given one-hot encoded node states $x_i^t \in \{0, 1\}^M$, where $M$ is the total number of  states, we apply a linear projection in $\mathbb{R^\text{D}}$ with operator $\M{U} \in \mathbb{R^{\text{D}\times\text{M}}}$. \nd{what is D here? Is this a fully connected neural net mixing multiple nodes? I don't think we do that.} \cs{It is a fully connected layer (refer to eq 9), but it is not mixing node features - it is per node and is projecting it into D dim}
%
% \begin{equation}
%     \V{h_{i}^{0}} = U^{0}m_i
% \end{equation}
%
We  take the projections and apply $L$ layers of Graph Convolutional Network (GCN). In general, a GCN represents a functional mapping  by $g(A, \V{h}) = a( f(A)\cdot \V{h}+ \V{b})$, with $A$ being the graph adjacency matrix and $a$ being the activation function. 
\nd{You are missing the weights}
For instance, for a GCN with symmetrized adjacency matrix, $f(A)= D^{-1/2}AD^{-1/2}$  \ry{for GAT} The authors of GCN suggest addition of self-loops such that $\hat{A} = A + I$ to ensure that the features of the central node $h_i^l$ are accounted for in layer $l + 1$. We sidestep this issue by using residual connections between GCN layers and notice a significant lift in model performance.
%
\begin{align}
  \V{h}_{i}^{0} = \M{U}^{0}x_i^t, \quad   \V{h}_{i}^{l+1} = \V{h}_{i}^{l} + \sigma(\texttt{BN}(g(\V{h}_i^l)), \quad 
      {y_i} = \V{P} \texttt{ReLU}(\V{Q}\V{h_i^L})t
\label{eqn:gcn_design}
\end{align}
%
Given the learned representation $\V{h}_i$, we  use a set of readout layers parameterized by $\V{Q} \in \mathbb{R}^{D\times D}$  and $\V{P} \in \mathbb{R}^{1 \times D}$ to generate   $y_i \in \mathbb{R}$,  which represents the probability that node $i$ being patient zero.


\section{Backup 2020-05-28}


\subsection{Difficulty of finding Patient Zero}
The task of finding P0 % requires learning the backward dynamics. 
% This task 
is compounded by the stochasticity of the infection spreading, resulting in different outcomes from the same initial conditions. 
We examine the possibility of establishing bounds on identifiability of P0 using a GCN-based model in in SIR-like dynamics on graphs. 
The main factors which affecting the ability to predict P0 are: (1) Ambiguity of patient zero; (2) Spreading radius of the infection relative to the diameter of the graph; (3) The parameters and type of the underlying epidemic model. 
% \begin{enumerate}
%     \item Ambiguity of patient zero,
%     \item Diameter of the graph, 
%     \item Spreading radius of the infection. 
%     \item The parameters and type of the underlying epidemic spreading model. \cs{Should we also mention dynamics of the underlying spread governed by $\beta$, $\gamma$}?
% \end{enumerate}
The ambiguity of P0 is due to some nodes being indistinguishable from each other, such as leaf nodes in a tree. 
The diameter, which is the maximum shortest distance between any pair of nodes, will affect how deep our GCN-based model needs to be in order to reach all potential P0. 
The spreading radius depends on the time passed since P0 as well as the parameters of the dynamics.
Combined with its upper boud, the graph diameter, the spreading radius will set a lower bound on the depth of the GCN model. 
Below, we explain how each of these factors plays a role and try to estimate their effect on identifying P0. 

\subsection{Graph Isomorphism and Ambiguity of Patient Zero}
\begin{wrapfigure}{r}{0.6\textwidth}
% \includegraphics[width=.5\linewidth]{figs/hash-infected-subgraph138-BA-5-k_max200.pdf}
\includegraphics[width=.49\linewidth]{figs/hash-infected-subgraph100-RGG-200-k_max5.pdf}
\includegraphics[width=.49\linewidth]{figs/hash-infected-subgraph115-BA-200-k_max5.pdf}
\caption{Equivalence classes of the quick hashing method inspired by the Weisfeiler-Lehman algorithm. 
Grey nodes are outside of the infected subgraph $G_I$. 
The colors indicate the equivalence classes. On the tree (right) $G_I$ has 115 nodes, but only $38$ distinct equivalence groups.
The Random Geometric Graph (left), however, with 100 infected nodes has 84 distinct groups. 
}
\label{fig:Ambiguity}
\vspace{-3mm}
\end{wrapfigure}
%
Compared to a random walk, epidemic spreading is more identifiable, as visited sites will change from the S state to a different state. 
\nd{ambiguity rooted in GI} 
% For the SI model (i.e. SIR with $\gamma=0$, meaning no recovery) concrete results have been for trees using ``rumor centrality'' \cite{shah2011rumors}. 
% Rumor centrality measures the closeness centrality of infected nodes to the last nodes being infected and the most central node is shown to be a maximum likelihood estimator for P0 on trees. 
% Closeness centrality ranks the node by $\sum_j 1/d_{ij} $ where $d_{ij}$ is the graph distance between $i,j$, the intuition being that P0 should have a balanced distance from the boundary of the spreading.
% For instance, in SI over a grid, the infection will look roughly circular after a long time and P0 is at the center of the circle. 
However, it may happen that the problem of finding P0 is unidentifiable 
when some nodes in the graph are identical. 
\ry{separate the analyze of trees and general graphs}
For instance, in a tree, if P0 is predicted to be a leaf, all leaves sharing the same parent are equally likely to be P0 \ry{this only happens if we have multiple patient zeros} \nd{no, even for a single P0, it's ambiguous.}. 
If some nodes are truly indistinguishable, 
%then an algorithm which predicts any of them as P0 is giving the right answer. 
our measure of accuracy should check P0 modulo an equivalence relations between nodes, i.e. automorphisms of the graph. 
% In such cases, we need to assess the accuracy of our prediction by grouping equivalent nodes together. 
% This equivalence is related to ``graph canonication'' and the graph isomorphism problem. 
We want to find nodes in the infected subgraph ${G}_I\subset {G}$ which can be mapped to each other via an element of the automorphism group $Q = \mathrm{Aut}({G}_I) \subset {G}$. \ry{this should come first}
% Consider a random walk on a star-shaped graph, which has one root node $v_0$ and $N-1$ leaf nodes $v_i$ and all edges are undirected, connecting only $v_0$ to $v_i$. 
% Let $x^t = (x_0^t,...x_{N-1}^t)$ represent the state of the walk on the graph at time $t$. 
% $x_i^t=1$ if the walker is at node $i$ at time $t$ and zero otherwise. 
% The probability of a state $x^t$ is given by 
% \begin{equation}
%     P(x_i^t=1|x_j^{t-1}) = \delta_{j0}(1-\delta_{i0}) + (1-\delta_{j0})\delta_{i0} 
% \end{equation}
% where the Kronecker delta $\delta_{ij}$ is $1$ if $i=j$ and zero otherwise. 
% Clearly, if at $ t=2$ the walker is not at the root node, it could have been in any of the leaf nodes at $t=0$. 
% Suppose we try to predict the $t=0$ position of the walker using machine learning. 
% In a naive approach, we would use the $t=2$ as input and ask the algorithm to return the precise index of the node at $t=0$. 
% This not only results in a performance equal to a random prediction (except never picking the root node), but may also lead to the model fitting the sampling noise. 
%
% The ambiguity described above is due to the fact that many nodes are equivalent to each other under certain dynamical processes on the graph.
% In the star graph above, any of the $(N-1)!$ shuffling of the leaf nodes looks exactly the same to the random walk. 
% These shuffling all result in graphs isomorphic to the original $G$ and constitute the automorphism group $\mathrm{Aut}(G)$. 
% In general, the set of nodes that are equivalent for a dynamical process can be mapped to each other using a subgroup $Q\subset  \mathrm{Aut}(G)$. 
Finding $\mathrm{Aut}(G_I)$ is relate to the Graph Isomorphism (GI) problem, which is a problem in NP, but not known whether or not it is NP-complete \cite{mckay1981practical}.
% To measure accuracy of finding P0, we need to group equivalent nodes under $\mathrm{Aut}(G_I)$. 
There exist many algorithms for GI \cite{MCKAY201494}, all of which are at least exponential in $N$. 
% Our goal of finding equivalent nodes under the action of $\mathrm{Aut}(G)$, is related to finding the graph invariant known as the canonical form, which in general can be as hard as GI.
We choose to use a simpler heuristic inspired by the Weisfeiler-Lehman (WS) graph kernel \cite{weisfeiler1968reduction, shervashidze2011weisfeiler}. 
The idea is to label the nodes by a sequence of numbers encoding the local structure of the graph around each node. 
A simple aggregate measure for this is % number of paths $p_i^l$ of a given length $l$ starting from each node $i$.
% Since paths include repetitive movements, a better measure would be 
the number nodes $n_i^{(l)}$ within a distance $l$ from node $i$. 
% Using this walk-based approach, 
Hence, we can label each node by the sequence $n_i =(n_i^{(1)},...,n^{(l_{\max})}_i) $.  
$n_i^{(1)}$ is the degree of node $i$ and we have $n_i^{(l)} = \theta(A_I^l) \mathbf{1}$
% \begin{equation}
%     n_i^l = \theta(A^l) \mathbf{1} \label{eq:nil}
% \end{equation}
with $A_I^l$ being the $l$th power of the adjacency matrix of the $G_I$ and $\theta(\cdot)$ the step function. % $\theta(x) = \{1, \mbox{ if} x>0; 0,\mbox{else}\} $ 
Figure \ref{fig:Ambiguity} shows that on trees there are many equivalent nodes, even non-leaf nodes.
However, the structure of contact networks where diseases spread is much more localized. A good proxy for contact networks is a Random Geometric Graph (RGG). 
Left of Figure \ref{fig:Ambiguity} shows that on RGG, the level of node equivalence is far less, with most nodes being distinguishable. 
In general, we find non-tree graphs with sufficient randomness (e.g. RGG and random graphs), there are very few equivalent nodes in small graphs. 
Hence, we neglect we believe in realistic settings this ambiguity won't play a major role in detectability of P0.  
\nd{but on tree BA we should definitely group nodes.}


% \subsection{Identifiability of Patient Zero}




In short, the fraction of triangles per connected triplet is $p$. 
In the worst case, $G_I$ grows as BFS, leading to $|G_I|\sim R_0t$. 
The probability of a connected triplet of nodes making a triangle (the ``clustering coefficent'') is $C= {n\choose 3}p^3/{n\choose 3} p^2 = p$. 
The probability of loops longer than triangles is smaller, so we focus on triangles. 
Hence, in a connected ER, $C> 2\log N /N$.

When $R_0>1$, at every time step an average of $R_0$ new infection are added to the infection graph $G_I$, meaning $|G_I| \sim R_0 t$.
When multiple infections are added, from one node, the infection spreads as a breadth-first search (BFS), so the breadth grows as $R_0t$.  
The depth of the infection graph can only increase by one at each infection step, so the depth first growth of $G_I$ is with $t$.
Thus, the lower bound on the number of triangles $n_{tri}$ can be found from the depth of $G_I$ 
\begin{equation}
    n_{tri} > 2(t-2){\log N\over N}
\end{equation} 
% In the other extreme, if the infection spreads as a star (breadth-first search, BFS), 
The breadth of $G_I$ yields the upper bound. 
For every parent infected node, every new child is connected to all the previously infected children. 
In the extreme case where $|G_I|\sim R_0t$ grows as a star-shaped network, we get the maximum potential triplets of nodes ${|G_I|-1\choose 2} \sim O(|G_I|^2)$ to make triangles, yielding the upper bound
\begin{equation}
    n_{tri} < 2{|G_I|-1 \choose 2} {\log N\over N} \sim R_0^2 t^2 {\log N\over N} 
\end{equation}
Thus, we expect 
\begin{equation}
    O(R_0^2t^2) > n_{tri} {N\over \log N} > O(R_0t)
\end{equation}
in a connected random graph. 
With each triangle, we expect the probability of correctly identifying P0 to fall by the number of ambiguous choices. 
A node which is infected can infect its neighbors as long as it is in the $I$ state. 
Therefore, the infection does perform a BFS, until a node enters the $R$ state
Therefore, we expect finding P0 to become difficult after $t_{tri}$ when the expected number of triangles with BFS becomes $n_{tri}>1$, meaning
\begin{align}
    % t_1 &\sim {N\over R_0 \log N}, & 
    t_{tri} &\sim {1\over R_0}\sqrt{{N\over \log N}}. \label{eq:t_tri-BFS0}
\end{align}
The computation is different for graphs different than a random graph, but the general idea is that when loops appear in the infection graph, inferring P0 can become ambiguous and difficult.  


Another simple heuristic for when loops appear in $G_I$ is when $|G_I|\sim O(N)$.
Using \eqref{eq:I(t)-epidemic}, assuming the exponential growth persists as long as $G_I$ is a tree, we get 
\begin{align}
    \sum_i I_i(t_{\max}) &\sim N, & 
    \Rightarrow t_{\max} &\sim {\log N \over \beta \lambda - \gamma} = {\log N \over \gamma (R_0 - 1)} 
    \label{eq:t_max-gamma}
\end{align} 
% Another heuristic for when the loops will be encountered is when the infection graph grows to the diameter of the graph, i.e. the maximum of the shortest distance between any two nodes. 
% At this point, the chance of making loops increases dramatically  all the shortest paths between any two node have 

%but in general, the more star-shaped they are, the worse it will be. 
% For example, the Barabasi-Albert graph with minimum degree $m>1$ has hubs which make the network mostly star-shaped. 
% While the number of triangles in these graphs is very small, we still expect loops to appear with $n_{tri} \sim O(R_0^2 t^2)$ 


\nd{Todo: 1) refer to Zaman-Shah to say tree-like infection network easy and solved; 2) estimate $t_{\max}$ where encountering many loops becomes probable; 3) relate $t$ to time of diffusion and distance from P0; 4) make the entropy argument (forward more infections than backward); 6) calculate explicit formulas for $t_{\max}$, once for exponential growth, once linear. }
However, combinatorically, the problem should be very challenging, since in every MP step we need to include the new neighbors of each node to find who could have infected it, resulting in an exponentially growing set for P0 similar to the forward dynamics \eqref{eq:I(t)-epidemic}.
In general, if the infection had taken over most of the graph, with $|G_I|\sim O(N)$,  
we would have to deal with an exponentially growing set of candidate nodes as we moved backwards in time and finding P0 would be difficult. 
However, if the infection is still in early stages and $|G_I|\ll N$, we can argue that finding P0 should be tractable. 
To illustrate, consider random graphs, where the leading eigenvalue is roughly the average degree $\lambda_1 \approx \bk{d}$. 
With $R_0 = \beta \bk{d}/\gamma > 1$,
% we have an epidemic. 
% Since the spreading probability from each node $j$ to its neighbor $i$ is given by $\beta {A}_{ij} p_j$, if $ d_j > 1$, 
% the size of the infection grows over time, if the number of infected nodes is much smaller than the total number of nodes, meaning $|G_I|\ll N$. 
% In this situation, 
in early stages the number of infections grows exponentially as in \eqref{eq:I(t)-epidemic}. 
This produces an asymmetry between the forward and backward dynamics. 
In particular, when $R_0 \ll \bk{d_i}$ the number of nodes that can potentially have infected node $i$ is a small subset of its neighbors. 
Hence in random graphs when $|G_I| \ll N $, in every backward MP step infector nodes get at least $R_0$ messages, whereas receivers of infectious signals on average had only one infected neighbor.
Since $R_0>0$, this reinforcement of the MP signals on earlier infectors will shrink set of P0 candidates exponentially, making it tractable to make a prediction. 
Note that, after contagion, where $|G_I|\sim O(N)$ or if the the size of P0$\sim O(N)$, this asymmetry between forward and backward dynamics disappears and it should be difficult to find P0. 
In particular, if the diameter $G_I$ becomes the diameter of $G$, most likely we have $|G_I|\sim O(N)$. 
From \eqref{eq:I(t)-epidemic}, this can happen when $t_{\max{}}(\beta \lambda_1 - \gamma) \sim 1$. 
We expect the inference problem to see a sharp drop in accuracy around $t_{\max{}}$
\nd{Can we test this? Do we see the oppsite? }

% \nd{Derive the duality under $S \leftrightarrow I$ in the SI model. Relate that to SIR. Talk about entropy conditions. }

% \ry{this says nothing about the learnability of the backward dynamics} 

% \ry{I don't understand what is the theoretical take-away here}


\section{Backup 2020-05-18}
We now present our theoretical analysis for the identification conditions. 
%
Assume that we have graph $G(V,E)$ with $N = |V|$ vertices labeled by indices $i \in \{1,\cdots, N\} $ and edge set $E$ captured by the adjacency matrix entries $A_{ij}$ which are nonzero if $ i$ is connected to $j$. 
We will mostly focus of undirected (i.e. $A_{ij} = A_{ji}$), unweighted graphs, though our results do not depend on this assumption. 
Consider a Markovian network (graph) diffusion process where the probability $P(x_i^t= \mu)$ of node $i$ being in state $\mu\in \{S,I,...,R\} $ at time $t$ only depends on the probabilities at $t-1$. 
For brevity, define $p_{i}^\mu(t) \equiv P(x_i^t= \mu) $. % each node $i$ can be in a number of states $\mu $ (e.g. $S,I,R$) at time $t$ 
In a network diffusion process the assumption is that node $i$ can only be directly affected by state of node $j$ if there is a connection between them, i.e. if $A_{ij} \ne 0$. 
This restriction means that the diffusion process is \textit{not} a general function of $p_i^\mu$, \ry{what is $f(p)$ here?} \nd{$f(p)$ mixes node features while preserving node index. It is some nonlinear function acting on the probabilities before they are used in diffusion. } but rather one restricted by the graph structure
\out{
\begin{align}
    p_i^\mu(t+1) &= F(A;p(t))_i^\mu 
    = f\pq{ \sum_j f_A(A)_{ij} f_p(p_j(t))^\mu   }  
\end{align}
where $f_A(A)_{ij}$ is only nonzero when $A_{ij}$ is nonzero, and $f_p(p_i)$ can mix the states $\mu$ but does not change the node index $i$. 
These functions can be expressed as 
\begin{align}
    f_A(A)_{ij} &= \theta(A_{ij}) \tilde{f}(A)_{ij} &
    f_p(p_i)^\mu = \sigma\pq{\sum_\nu W^\mu_\nu p_i^\nu + b^\mu}
    \label{eq:f_pA}
\end{align}
}%
\nd{empirical distrbution} 
\begin{align}
    F_a(A;p)_i^\mu &\equiv \sum_{j} f_a\Big( g_a(A)_{ij} h_a(p_j)^\mu \Big)
    \label{eq:gen_diff_F} \\
    p_i^\mu(t+1) &= F(A;p(t))_i^\mu 
    = \sigma \pq{ \left\{ F_a(A;p(t))^\mu_i \right\} } %\cr 
    \label{eq:gen_diffusion}
\end{align}
where $f_a$ may be any positive function, the index $a$ allows nonlinear mixing of different propagation rules the $g_a(A)_{ij}$, which are only nonzero when $A_{ij}$ is nonzero, and $h_a(p_i)$ can mix the states $\mu$ but do not change the node index $i$.  
These functions can be expressed as 
\begin{align}
    g_a(A)_{ij} &= \theta(A_{ij}) \tilde{g}_a(A)_{ij} &
    h_a(p_i)^\mu = \sigma_a\pq{\sum_\nu W^\mu_{a,\nu} p_i^\nu + b^\mu_a }
    \label{eq:gh_RD}
\end{align}
where $\theta(\cdot)$ is the step function and $\sigma_a(\cdot)$ a nonlinear function.
Dynamics of the form \eqref{eq:gen_diffusion} are a type of nonlinear Reaction-diffusion (RD) dynamics \nd{citation} defined on graphs and have been used to describe epidemic spreading \cite{colizza2007reaction}. 
% For example, simple diffusion on a graph, we have two states $S,I$ and diffusion is changing the $S\to I$ state. 
The probability $P_{ij}\equiv P(x_i^{t+1}=I| x_j^t=S)$ 
of node $i$ getting infected at $t+1$ given node $j$ was in the infected state at time $t$ is given by the diffusion operator $ \hat{A}_{ij} = [AD^{-1}]_{ij}$ where $D_{ij} = \delta_{ij} \sum_k A_{ik}$ is the degree matrix, because node $j$ is equally likely to infect any of its neighbors. 
% \nd{The correct one may be $AD^{-1}$ b/c $p_j$ may be spreading to all its neighbors equally, while $i$ is the receiver and just aggregates whatever is passed to it by its neighbors. }
The agent-based models \eqref{eq:SIR} and \eqref{eq:SEIR}, which correct for double-counting of infection from multiple neighbours, can be rewritten using the diffusion operator $ \hat{A}_{ij}$. 
The left part of \eqref{eq:SIR} may be modified and written in terms of likelihoods (Supp. \ref{ap:SIR-RD}) as $ p_i(t+1)^I  = p_i^S(t) P(x_i^{t+1}=I|x_i^t = S)$ 
and for small $\beta$ yield 
\begin{align}
    P(x_i^{t+1}=I|x_i^t = S) & = 1- \prod_{j} \pq{1-\beta \hat{A}_{ij}p_j^I} = \beta \sum_j \hat{A}_{ij}p_j^I - \beta^2 [\hat{A}p^I]^2% \sum_{j,k} \hat{A}_{ij} p_j \hat{A}_{ik}p_k 
    +O(\beta ^3)  
    \label{eq:p_i-expansion0}
\end{align}
which yields the simplified equation $ p_i(t+1)^I  = p_i^S(t) \sum_j \beta \hat{A}_{ij} p_j^I(t) $.
\eqref{eq:p_i-expansion0} both before and after expansion can be written in form of \eqref{eq:gen_diffusion} (Supp.  \ref{ap:SIR-RD}). 
The rest of SIR and SEIR equations do not involve the the graph adjacency $A$ at all, meaning $g_a(A)=I$, and $F_a(A;p)_i^\mu \propto p_i^\mu $. \ry{make the connection for back-ward dynamics}

\paragraph{Point-processes} 
We will be focusing on point-processes (e.g. random walk), instead of continuous diffusion, meaning that the diffusion also involves a stochastic sampling where out of the nodes with $p_i^I(t) >0 $ some will go into $x_i^t = I$ state and some won't. 
This can be encoded in \eqref{eq:gen_diffusion} by adding a sampling step, converting $p_i^\mu$ to discrete states $\tilde{p}_i^\mu =\mathcal{F}(p_i)^\mu $ which decides the state $x_i^t$ by taking into account all $p_i^\nu$ for being in states $\nu = S,I,...$. 
\nd{Markov chain complex; to make it simpler we work with mean-field approach i.e. probabilities. }

\paragraph{Relation to Graph Neural Networks}
In conclusion, the epidemic spreading models on graphs all fall under the umbrella of the reaction-diffusion equations \eqref{eq:gen_diffusion}. 
This has a strong implication on what machine learning methods could mimic the behavior of these systems efficiently. 
Specifically, we arrive at the following
\begin{proposition}
    A Reaction-diffusion system on a graph can be approximated using neural message-passing \cite{gilmer2017neural}, or graph convolutional networks \cite{kipf2016semi} with multiple propagation rules, residual connections and nonlinear aggregation function. 
\end{proposition}
The action of a graph convolutional network (GCN) \cite{kipf2016semi}, taking node features $h_i^\mu$ for node $i$ and feature channel $\mu$ as input, is given by 
\begin{align}
    F(A;h)^\mu_i & = \sigma\pq{\sum_j g(A)_{ij} \pq{h_j^\nu W_\nu^\mu + b^\mu } } 
\end{align}
Where we have allowed a bias term $b^\mu$.
The propagation rule (PR) $g(A)$ is generally chosen as $D^{-1/2} A D^{-1/2}$ in GCN, but other rules have also been employed in the literature. 
The main constraint on the PR is that information only moves along edges, hence $g(A)$ should satisfy \eqref{eq:gh_RD}. 
We may use multiple GCN models with different PR 
$g_a(A)$. 
The GCN aggregation function is a simple sum over the PR index $j$ contracted with the node features. 
However, general nonlinear aggregation as $f_a$ in \eqref{eq:gen_diff_F}, as well as nonlinear functions like $h_a$ in \eqref{eq:gh_RD} have also been used in the literature, such as neural message passing architectures  
\cite{gilmer2017neural}. 
Hence, RD dynamics has the same structure as neural message-passing and graph neural networks based on these architectures should be able to learn the forward RD dynamics.
\qed 

\subsection{Learning the Backward Dynamics}
We wish to see if we can learn the backward dynamics of \eqref{eq:gen_diffusion} to find patient zero. 
What can the forward dynamics teach us about learning the backward dynamics? 


\ry{this says nothing about the learnability of the backward dynamics} 
This suggests that the forward dynamics of graph diffusion processes could be efficiently learned using recurrent GCN-based models if time-series data is available. 

\ry{I don't understand what is the theoretical take-away here}


As we saw above, reaction-diffusion (RD) dynamics on graphs, including epidemic spreading models such as SIR, are a generalization of message passing.
They may be non-linear and even stochastic, but they are constrained by the graph structure and agnostic about which neighbor each node gets infected by.
Below, we will discuss how one can learn RD using machine learning.  



\subsection{Detection Probability}
We analyze the probability of accurately recover the diffusion source given  the diffusion dynamics. The technical difficulty of the analysis stems from the (1) the presence of cycles in graphs (higher-order transmission) (2) the recovery state introduces additional uncertainty to the diffusion process (3) the exact time step of the snapshot is unknown.
%
Existing theoretical results mostly focus on the SI dynamics without considering the removed state. For example, \cite{shah2011rumors} defines \textit{rumor centrality} to measure the probability of each node being the diffusion source. Intuitively, as the transmission is random, the infection sequences includes all possible permutations of the nodes, constrained by the topological order the order. Specifically, denote a  tree  of $N$ nodes with root  $u$ as $T_N(u)$, the  rumor centrality is defined as
\begin{equation}
    R(N,u)= N! \frac{1}{\prod_{v\in {T}_N(u)} |T_N(v)|}
\end{equation}

The following theorem guarantees the success probability of identifying patient zero for a regular tree with degree $d$:
\begin{theorem}
Let $T_n(n)$ be a diffusion on a d-regular tree with degree $d\geq 3$, for any $\eta \in (0,1)$ and $k \geq 3$, 
\[\lim\sup_{n\rightarrow \infty} \mathbb{P}(M = \mathcal{A}^\star  ) \geq  C_1 \eta^{\frac{d-1}{d-2}} + C_2 k^{\frac{2d-3}{d-2}}(1-\eta)^{k-1+\frac{1}{d-2}}\]
with $M$ being the estimator using rumor centrality.
\end{theorem}

\ry{Analyze using Galton–Watson process/Branching Process}
% https://www.cs.cornell.edu/home/kleinber/networks-book/networks-book-ch21.pdf
In a $d$-regular tree, each $x_i$ affects $d$ neighbours with probability $\beta$. Let us focus on a quantity called \textit{basic reproductive number}, $R$, which the expected number of new cases infected by a single individual. Clearly for trees, if $Rd > 1$, the disease will continue to be contagious with probability larger than zero. There will be at least one node in $\V{x}^t$ that is infected and we can easily identify patient zero. If $Rd < 1$, then with probability $1$, the disease with die out. The probability of identifying patient zero after the disease dies out is zero. 




\nd{
1) For binary graphs (degrees $d=3$) they predict a detection probability of $1/4$. Can you check if for $\gamma \to0$ or $\gamma \ll \beta $ GCN reaches this limit for high $t$?

2) How efficient is the rumor centrality compared to DMP and GCN? How does it scale with size of network?  
}


% Given a dataset of  graph snapshots $\{\V{x}^t\}$ from an SIR dynamics, we wish the obtain the estimator for the problem in \eqref{eqn:patient_zero}. 
% The general loopy graph is difficult to analyze, we limit our analysis to irregular trees. The following result states the existence of an estimator for finding patient zero:
% \begin{theorem}[Existence\cite{bubeck2017finding}]
% There exist constants $c$, $c'>0$ such that the following holds true in the ER graph. Any root-finding algorithm must satisfy $K(\epsilon) \geq \exp(\sqrt{c\log(1/\epsilon})$.
% Furthermore, there exists a polynomial time root-finding algorithm with $K(\epsilon) \leq  \exp( c'\frac{\log(1/\epsilon)}{\log \log(1/\epsilon)})$. Here $K(\epsilon)$ is output top $K$ nodes with accuracy $\epsilon$ to find patient zero.
% \end{theorem}

\subsection{Difficulty of finding Patient Zero}
Our goal is to learn patient zero $\mathcal{Z}$)\, i.e., where the spreading started, which requires learning the backward dynamics. 
Moreover, the task is compounded by the stochastic sampling step, resulting in many different outcomes starting from the same initial conditions. 
We wish to examine whether it is possible to establish approximate bounds on accuracy of a GCN-based model for learning patient zero in SIR-like reaction-diffusion dynamics on graphs. 
There are three main factors which affect our ability to predict P0:
\begin{enumerate}
    \item Ambiguity of patient zero,
    \item Diameter of the graph, 
    \item Spreading radius of the infection. 
    \item \cs{Should we also mention dynamics of the underlying spread governed by $\beta$, $\gamma$}?
\end{enumerate}
The ambiguity may be due to some nodes being equivalent to each other, such as leaf nodes in a tree or a star-shaped graphs. 
The diameter, which is the maximum shortest distance between any pair of nodes, will be related to how deep our GCN-based model needs to be. 
Finally, the spreading radius, which depends on the time passed since P0 as well as the parameters of the dynamics, combined with the graph diameter will set a lower bound on the depth of the GCN model. 
Below, we explain how each of these factors plays a role and try to estimate their effect on identifying P0. 


% \subsection{Identifiability of Patient Zero}
\subsection{Ambiguity of Patient Zero}

In the SI model, the task is slightly more identifiable than a random walk, as visited sites remain in the $I$ state, with concrete results derived for trees \cite{shah2011rumors}. 
The ``rumor centrality'' \cite{shah2011rumors} measures the closeness centrality of infected nodes to the last nodes being infected and the most central node is shown to be a maximum likelihood estimator for P0 on trees. 
At the core of this result is that P0 should have a balanced distance from the boundary of the spreading. 
For instance, in SI spreading over a grid, the infection will look roughly circular after a long time and P0 is at the center of the circle. 
However, it may happen that the problem of finding P0 is unidentifiable. 
For instance, in simple random walk on a grid finding the starting node is ill-defined.
After $t$ steps, any node within a distance $r$ has a likelihood of being the starting node with a probability proportional to $\exp[-r^2/2t]$, resulting in a ring-like distribution for likely P0's around the current position of the walker.  
Also, in the SIR-type dynamics where the infection leaves a trace, P0 may not be precisely identifiable when some nodes in the graph are identical. 

\ry{separate the analyze of trees and general graphs}
For instance, in a $k$-ary tree, if P0 is predicted to be at level $l$, and a few branches are infected the same amount, all level $l$ nodes on infected branches may be equally likely to be P0 \ry{this only happens if we have multiple patient zeros}. 
In such cases, we need to assess the accuracy of our prediction by grouping equivalent nodes together. 
This equivalence is related to ``graph canonication'' and the graph isomorphism problem. 
In effect, we want to find the nodes in the infected subgraph $\mathcal{S}\subset \mathcal{G}$ which can be mapped to each other so that we end up with an identical subgraph. 
These mappings constitute the automorphism group $\mathrm{Aut}(\mathcal{S})$ of the infected subgraph. \ry{this should come first}


Consider a random walk on a star-shaped graph, which has one root node $v_0$ and $N-1$ leaf nodes $v_i$ and all edges are undirected, connecting only $v_0$ to $v_i$. 
Let $x^t = (x_0^t,...x_{N-1}^t)$ represent the state of the walk on the graph at time $t$. 
$x_i^t=1$ if the walker is at node $i$ at time $t$ and zero otherwise. 
The probability of a state $x^t$ is given by 
\begin{equation}
    P(x_i^t=1|x_j^{t-1}) = \delta_{j0}(1-\delta_{i0}) + (1-\delta_{j0})\delta_{i0} 
\end{equation}
where the Kronecker delta $\delta_{ij}$ is $1$ if $i=j$ and zero otherwise. 
Clearly, if at $ t=2$ the walker is not at the root node, it could have been in any of the leaf nodes at $t=0$. 
Suppose we try to predict the $t=0$ position of the walker using machine learning. 
In a naive approach, we would use the $t=2$ as input and ask the algorithm to return the precise index of the node at $t=0$. 
This not only results in a performance equal to a random prediction (except never picking the root node), but may also lead to the model fitting the sampling noise. 

The ambiguity described above is due to the fact that many nodes are equivalent to each other under certain dynamical processes on the graph.
In the star graph above, any of the $(N-1)!$ shuffling of the leaf nodes looks exactly the same to the random walk. 
These shuffling all result in graphs isomorphic to the original $G$ and constitute the automorphism group $\mathrm{Aut}(G)$. 
In general, the set of nodes that are equivalent for a dynamical process can be mapped to each other using a subgroup $Q\subset  \mathrm{Aut}(G)$. 
Finding $\mathrm{Aut}(G)$ is relate to the Graph Isomorphism (GI) problem, which is a problem in NP, but not known whether or not it is NP-complete \cite{mckay1981practical}.
For our purpose of assessing the accuracy of finding patient zero, we need a way to group equivalent nodes, which are equivalence sets under a subset of $\mathrm{Aut}(G)$. 
There exist many algorithms for GI \cite{MCKAY201494}, all of which are at least exponential in $N$. 

Our goal of finding equivalent nodes under the action of $\mathrm{Aut}(G)$, is related to finding the graph invariant known as the canonical form, which in general can be as hard as GI.
We choose to use a simpler heuristic inspired by the Weisfeiler-Lehman (WS) graph kernel \cite{weisfeiler1968reduction, shervashidze2011weisfeiler}. 
The idea is to label the nodes by a sequence of numbers encoding the local structure of the graph around each node. 
A simple aggregate measure for this can be number of paths $p_i^l$ of a given length $l$ starting from each node $i$.
Since paths include repetitive movements, a better measure would be the number nodes $n_i^l$ within a distance $l$ from node $i$. 
Using this walk-based approach, we can label each node by the sequence $n_i =(n_i^1,...,n^{l_{\max}}_i) $.  
$n_i^1$ is the degree of node $i$ and in general we have 
\begin{equation}
    n_i^l = \theta(A^l) \mathbf{1} \label{eq:nil}
\end{equation}
using the Heaviside step function $\theta(x) = \{1, \mbox{ if} x>0; 0,\mbox{else}\} $ 

\subsection{Effect of Graph Diameter on Model Architecture}
The prominent feature of network diffusion is that it is Markovian and is only transmitted to first neighbors of each node, as in message-passing \nd{Review Neural Message Passing}, meaning $g_m(A)_{ij} \propto \theta(A_{ij})$. 
This puts a fundamental restriction on how diffusion spreads over the graph and how a GCN could find P0. 











Theoretical bounds on GCN-based architectures: 
\begin{itemize}
    \item Relation of depth with graph diameter: Can all nodes be reached? 
    \item Relation of depth with range of diffusion (as a function of $R_0$): How far can it have spread and is it causally possible to predict with $d$ layer GCN?
    \item Define node equivalence based of $R_0$: only nodes within a certain range can be equivalent. 
\end{itemize}



As the diffusion dynamics is Markovian,  the joint distribution can be factorized as   $P(\V{x}^{t+1}| \V{x}^t)$ governs the evolution of node states $\V{x}$. The following theorem guarantees the estimator using GNNs. 

\begin{theorem}
A graph neural network in the form of  can accurately estimate patient zero  with probability $\delta$, if the network..
\label{eqn:estimation}
\end{theorem}

% Denote a $N$- node graph as $G=(V, E)$, where $|V|=N$. The concatenation of node states at time step $t$ is denoted as $\V{x}^t \in \real^N$, every node $\V{x}_i$ can take three state: S(susceptible), I (infectious), R(recovery). The joint state space for $\V{x}$ is thus $3^N$.  
%  and the state transition matrix of the Markov chain is $P \in \real^{N\times N}$. We have the dynamics of the diffusion process as:
% \[\V{x}^{t+1} =  P\V{x}^{t}\]
% The graph structure imposes assumptions on $P$, meaning:
% \[P_{ij} = \begin{cases} 0 & A_{ij} =0\\
% p_{ij}>0 & \text{otherwise} \end{cases}\]
% here $A$ is the adjacency of the graph. 








\section{Backup 2020-05-01}
\section{Theoretical Analysis}

We now present our theoretical analysis for the identification conditions. 
%
Assume that we have graph $G(V,E)$ with $N = |V|$ vertices labeled by indices $i \in \{1,\cdot, N\} $ and edge set $E$ captured by the adjacency matrix entries $A_{ij}$ which are nonzero if $ i$ is connected to $j$. 
We will mostly focus of undirected (i.e. $A_{ij} = A_{ji}$), unweighted graphs, though our results do not depend on this assumption. 
Consider a Markovian network (graph) diffusion process where the probability $P(x_i^t= \mu)$ of node $i$ being in state $\mu\in \{S,I,...,R\} $ at time $t$ only depends on the probabilities at $t-1$. 
For brevity, define $p_{i}^\mu(t) \equiv P(x_i^t= \mu) $. % each node $i$ can be in a number of states $\mu $ (e.g. $S,I,R$) at time $t$ 
In a network diffusion process the assumption is that node $i$ can only be directly affected by state of node $j$ if there is a connection between them, i.e. if $A_{ij} \ne 0$. 
This restriction means that the diffusion process is \textit{not} a general function of $p_i^\mu$, \ry{what is $f(p)$ here?} \nd{$f(p)$ mixes node features while preserving node index. It is some nonlinear function acting on the probabilities before they are used in diffusion. } but rather one restricted by the graph structure



\out{
\begin{align}
    p_i^\mu(t+1) &= F(A;p(t))_i^\mu 
    = f\pq{ \sum_j f_A(A)_{ij} f_p(p_j(t))^\mu   }  
\end{align}
where $f_A(A)_{ij}$ is only nonzero when $A_{ij}$ is nonzero, and $f_p(p_i)$ can mix the states $\mu$ but does not change the node index $i$. 
These functions can be expressed as 
\begin{align}
    f_A(A)_{ij} &= \theta(A_{ij}) \tilde{f}(A)_{ij} &
    f_p(p_i)^\mu = \sigma\pq{\sum_\nu W^\mu_\nu p_i^\nu + b^\mu}
    \label{eq:f_pA}
\end{align}
}%
\nd{empirical distribution} 
\begin{align}
    F_m(A;p)_i^\mu &\equiv \sum_{j} g_m(A)_{ij} f_m(p_j)^\mu 
    \label{eq:gen_diff_F} \\
    p_i^\mu(t+1) &= F(A;p(t))_i^\mu 
    = \sigma \pq{ \left\{ F_m(A;p(t))^\mu_i \right\} } %\cr 
    \label{eq:gen_diffusion}
\end{align}
where the index $m$ allows nonlinear mixing of different propagation rules the $g_m(A)_{ij}$, which are only nonzero when $A_{ij}$ is nonzero, and $f_m(p_i)$ can mix the states $\mu$ but do not change the node index $i$.  
These functions can be expressed as 
\begin{align}
    g_m(A)_{ij} &= \theta(A_{ij}) \tilde{g}_m(A)_{ij} &
    f_m(p_i)^\mu = \sigma_m\pq{\sum_\nu W^\mu_{m,\nu} p_i^\nu + b^\mu_m }
    \label{eq:f_pA}
\end{align}
where $\theta(\cdot)$ is the step function and $\sigma(\cdot)$ a nonlinear function.
For example, simple diffusion on a graph, we have two states $S,I$ and diffusion is changing the $S\to I$ state. 
The probability $P_{ij}\equiv P(x_i^{t+1}=I| x_j^t=S)$ of node $i$ getting infected at $t+1$ given node $j$ was in the infected state at time $t$ is given by the diffusion operator $ \hat{A}_{ij} = [D^{-1}A]_{ij}$ as $P_{ij} = \beta \hat{A}_{ij}$ where $D_{ij} = \delta_{ij} \sum_k A_{ik}$ is the degree matrix. \nd{The correct one may be $AD^{-1}$ b/c $p_j$ may be spreading to all its neighbors equally, while $i$ is the receiver and just aggregates whatever is passed to it by its neighbors. }
The infection probability is given by $p_i^I(t+1) = \beta \hat{A}_{ij} p_j^I(t)$ and $p_i^S = 1-p_i^I$. 
Hence, for diffusion $g_1(A) = \beta \hat{A}$ and $f_1(p_j)^\mu = \sum_{\nu}  \delta^\mu_I \delta^I_\nu p^\nu_j$. 
In regular diffusion there is no condition on the target node $i$ and even if it is in the $I$ state the dynamics is the same.
In the SI model, however, the infection only spreads to $i$ if it is in the $S$ state. 
Thus, we have to multiply the dynamics by $p_i^S \equiv P(x_i^t = S)$ which yields
\begin{equation}
    p_i^I(t+1) = \beta \hat{A}_{ij} p_j^I(t) p_i^S.  
    \label{eq:SI}
\end{equation}
This can still be written as \eqref{eq:gen_diffusion} by adding the extra functions $g_2(A) = I$ (identity matrix) and $f_2(p_j)^\mu = \sum_\nu  \delta^\mu_S  \delta^S_\nu p^\nu_j$ and having 
\begin{align}
    p_i(t+1)^I =%\prod_{m\in \{1,2\} } 
    F_m(A;p(t))_i^I F_2(A;p(t))_i^S 
\end{align}
where $F_m = g_m\cdot f_m $  are as in \eqref{eq:gen_diff_F}. 
More complex epidemic spreading models such as SIR and SEIR can also be written in a similar fashion. 
In SIR and SEIR the rest of the dynamic equations are linear and do not involve the the graph adjacency $A$ at all, meaning $g_m(A)=I $  in the rest of the equations. 
Lastly, note that $\beta \sum_j\hat{A}_{ij} p_j $ can exceed 1, rendering \eqref{eq:SI} inconsistent with $p_i^I$ being probabilities.  
More realistically, we would have to correct for double-counting of infection signals coming from different neighbors and have  
\begin{align}
    p_i(t+1)^I & \propto 1- \prod_{j\in \partial_i } \pq{1-\beta \hat{A}_{ij}p_j^I} 
    = \beta \sum_j \hat{A}_{ij}p_j - \beta^2 \sum_{j,k} \hat{A}_{ij} p_j \hat{A}_{ik}\cdot p_k + O(\beta ^3) 
\end{align}

We will be focusing on point-processes (e.g. random walk), instead of continuous diffusion, meaning that the diffusion also involves a stochastic sampling process where out of the nodes with $p_i^I(t) >0 $ some will go into $x_i^t = I$ state and some won't. 
This can be encoded in \eqref{eq:gen_diffusion} by adding a sampling step, converting $p_i^\mu$ to discrete states $\tilde{p}_i^\mu =\mathcal{F}(p_i)^\mu $ which decides the state $x_i^t$ by taking into account all $p_i^\nu$ for being in states $\nu = S,I,...$. \ry{I don't understand what is the theoretical take-away here}
\nd{This part was still evolving. The main take-away was the structure of reaction-diffusion equations on graphs is a generalized message passing and like GCN }. 

As we saw above, reaction-diffusion (RD) dynamics on graphs, including epidemic spreading models such as SIR, are a generalization of message passing.
They may be non-linear and even stochastic, but they are constrained by the graph structure and agnostic about which neighbor each node gets infected by.
Below, we will discuss how one can learn RD using machine learning.  



\subsection{Detection Probability}
We analyze the probability of accurately recover the diffusion source given  the diffusion dynamics. The technical difficulty of the analysis stems from the (1) the presence of cycles in graphs (higher-order transmission) (2) the recovery state introduces additional uncertainty to the diffusion process (3) the exact time step of the snapshot is unknown.
%
Existing theoretical results mostly focus on the SI dynamics without considering the removed state. For example, \cite{shah2011rumors} defines \textit{rumor centrality} to measure the probability of each node being the diffusion source. Intuitively, as the transmission is random, the infection sequences includes all possible permutations of the nodes, constrained by the topological order the order. Specifically, denote a  tree  of $N$ nodes with root  $u$ as $T_N(u)$, the  rumor centrality is defined as
\begin{equation}
    R(N,u)= N! \frac{1}{\prod_{v\in {T}_N(u)} |T_N(v)|}
\end{equation}

The following theorem guarantees the success probability of identifying patient zero for a regular tree with degree $d$:
\begin{theorem}
Let $T_n(n)$ be a diffusion on a d-regular tree with degree $d\geq 3$, for any $\eta \in (0,1)$ and $k \geq 3$, 
\[\lim\sup_{n\rightarrow \infty} \mathbb{P}(M = \mathcal{A}^\star  ) \geq  C_1 \eta^{\frac{d-1}{d-2}} + C_2 k^{\frac{2d-3}{d-2}}(1-\eta)^{k-1+\frac{1}{d-2}}\]
with $M$ being the estimator using rumor centrality.
\end{theorem}

\ry{Analyze using Galton–Watson process/Branching Process}
% https://www.cs.cornell.edu/home/kleinber/networks-book/networks-book-ch21.pdf
In a $d$-regular tree, each $x_i$ affects $d$ neighbours with probability $\beta$. Let us focus on a quantity called \textit{basic reproductive number}, $R$, which the expected number of new cases infected by a single individual. Clearly for trees, if $Rd > 1$, the disease will continue to be contagious with probability larger than zero. There will be at least one node in $\V{x}^t$ that is infected and we can easily identify patient zero. If $Rd < 1$, then with probability $1$, the disease with die out. The probability of identifying patient zero after the disease dies out is zero. 




\nd{
1) For binary graphs (degrees $d=3$) they predict a detection probability of $1/4$. Can you check if for $\gamma \to0$ or $\gamma \ll \beta $ GCN reaches this limit for high $t$?

2) How efficient is the rumor centrality compared to DMP and GCN? How does it scale with size of network?  
}


Given a dataset of  graph snapshots $\{\V{x}^t\}$ from an SIR dynamics, we wish the obtain the estimator for the problem in \eqref{eqn:patient_zero}. 
The general loopy graph is difficult to analyze, we limit our analysis to irregular trees. The following result states the existence of an estimator for finding patient zero:
\begin{theorem}[Existence\cite{bubeck2017finding}]
There exist constants $c$, $c'>0$ such that the following holds true in the ER graph. Any root-finding algorithm must satisfy $K(\epsilon) \geq \exp(\sqrt{c\log(1/\epsilon})$.
Furthermore, there exists a polynomial time root-finding algorithm with $K(\epsilon) \leq  \exp( c'\frac{\log(1/\epsilon)}{\log \log(1/\epsilon)})$. Here $K(\epsilon)$ is output top $K$ nodes with accuracy $\epsilon$ to find patient zero.
\end{theorem}
\subsection{Relation to Graph Neural Networks}
Dynamics of the form \eqref{eq:gen_diffusion} are a type of nonlinear Reaction-diffusion \nd{citation} defined on graphs and have been used to describe epidemic spreading \cite{colizza2007reaction}. 
We wish to see if we can learn the backward dynamics of \eqref{eq:gen_diffusion}. 
We note that the forward dynamics \eqref{eq:gen_diffusion} has the structure of a general graph neural network (GNN). 
Moreover, the restriction that $g_m(A)_{ij}$ be nonzero and usually proportional to $\hat{A} = D^{-1}A$ reduces the GNN to a Graph Convolutional Network (GCN) \cite{kipf2016semi}. \ry{this says nothing about the learnability of the backward dynamics} 
This suggests that the forward dynamics of graph diffusion processes could be efficiently learned using recurrent GCN-based models if time-series data is available. 

\subsection{Difficulty of finding Patient Zero}
Our goal is to learn patient zero $\mathcal{Z}$)\, i.e., where the spreading started, which requires learning the backward dynamics. 
Moreover, the task is compounded by the stochastic sampling step, resulting in many different outcomes starting from the same initial conditions. 
We wish to examine whether it is possible to establish approximate bounds on accuracy of a GCN-based model for learning patient zero in SIR-like reaction-diffusion dynamics on graphs. 
There are three main factors which affect our ability to predict P0:
\begin{enumerate}
    \item Ambiguity of patient zero,
    \item Diameter of the graph, 
    \item Spreading radius of the infection. 
    \item \cs{Should we also mention dynamics of the underlying spread governed by $\beta$, $\gamma$}?
\end{enumerate}
The ambiguity may be due to some nodes being equivalent to each other, such as leaf nodes in a tree or a star-shaped graphs. 
The diameter, which is the maximum shortest distance between any pair of nodes, will be related to how deep our GCN-based model needs to be. 
Finally, the spreading radius, which depends on the time passed since P0 as well as the parameters of the dynamics, combined with the graph diameter will set a lower bound on the depth of the GCN model. 
Below, we explain how each of these factors plays a role and try to estimate their effect on identifying P0. 


% \subsection{Identifiability of Patient Zero}
\subsection{Ambiguity of Patient Zero}

In the SI model, the task is slightly more identifiable than a random walk, as visited sites remain in the $I$ state, with concrete results derived for trees \cite{shah2011rumors}. 
The ``rumor centrality'' \cite{shah2011rumors} measures the closeness centrality of infected nodes to the last nodes being infected and the most central node is shown to be a maximum likelihood estimator for P0 on trees. 
At the core of this result is that P0 should have a balanced distance from the boundary of the spreading. 
For instance, in SI spreading over a grid, the infection will look roughly circular after a long time and P0 is at the center of the circle. 
However, it may happen that the problem of finding P0 is unidentifiable. 
For instance, in simple random walk on a grid finding the starting node is ill-defined.
After $t$ steps, any node within a distance $r$ has a likelihood of being the starting node with a probability proportional to $\exp[-r^2/2t]$, resulting in a ring-like distribution for likely P0's around the current position of the walker.  
Also, in the SIR-type dynamics where the infection leaves a trace, P0 may not be precisely identifiable when some nodes in the graph are identical. 

\ry{separate the analyze of trees and general graphs}
For instance, in a $k$-ary tree, if P0 is predicted to be at level $l$, and a few branches are infected the same amount, all level $l$ nodes on infected branches may be equally likely to be P0 \ry{this only happens if we have multiple patient zeros}. 
In such cases, we need to assess the accuracy of our prediction by grouping equivalent nodes together. 
This equivalence is related to ``graph canonication'' and the graph isomorphism problem. 
In effect, we want to find the nodes in the infected subgraph $\mathcal{S}\subset \mathcal{G}$ which can be mapped to each other so that we end up with an identical subgraph. 
These mappings constitute the automorphism group $\mathrm{Aut}(\mathcal{S})$ of the infected subgraph. \ry{this should come first}


Consider a random walk on a star-shaped graph \ry{what is the difference from a tree}, which has one root node $v_0$ and $N-1$ leaf nodes $v_i$ and all edges are undirected, connecting only $v_0$ to $v_i$. 
Let $x^t = (x_0^t,...x_{N-1}^t)$ represent the state of the walk on the graph at time $t$. 
$x_i^t=1$ if the walker is at node $i$ at time $t$ and zero otherwise. 
The probability of a state $x^t$ is given by 
\begin{equation}
    P(x_i^t=1|x_j^{t-1}) = \delta_{j0}(1-\delta_{i0}) + (1-\delta_{j0})\delta_{i0} 
\end{equation}
where the Kronecker delta $\delta_{ij}$ is $1$ if $i=j$ and zero otherwise. 
Clearly, if at $ t=2$ the walker is not at the root node, it could have been in any of the leaf nodes at $t=0$. 
Suppose we try to predict the $t=0$ position of the walker using machine learning. 
In a naive approach, we would use the $t=2$ as input and ask the algorithm to return the precise index of the node at $t=0$. 
This not only results in a performance equal to a random prediction (except never picking the root node), but may also lead to the model fitting the sampling noise. 

The ambiguity described above is due to the fact that many nodes are equivalent to each other under certain dynamical processes on the graph.
In the star graph above, any of the $(N-1)!$ shuffling of the leaf nodes looks exactly the same to the random walk. 
These shuffling all result in graphs isomorphic to the original $G$ and constitute the automorphism group $\mathrm{Aut}(G)$. 
In general, the set of nodes that are equivalent for a dynamical process can be mapped to each other using a subgroup $Q\subset  \mathrm{Aut}(G)$. 
Finding $\mathrm{Aut}(G)$ is relate to the Graph Isomorphism (GI) problem, which is a problem in NP, but not known whether or not it is NP-complete \cite{mckay1981practical}.
For our purpose of assessing the accuracy of finding patient zero, we need a way to group equivalent nodes, which are equivalence sets under a subset of $\mathrm{Aut}(G)$. 
There exist many algorithms for GI \cite{MCKAY201494}, all of which are at least exponential in $N$. 

Our goal of finding equivalent nodes under the action of $\mathrm{Aut}(G)$, is related to finding the graph invariant known as the canonical form, which in general can be as hard as GI.
We choose to use a simpler heuristic inspired by the Weisfeiler-Lehman (WS) graph kernel \cite{weisfeiler1968reduction, shervashidze2011weisfeiler}. 
The idea is to label the nodes by a sequence of numbers encoding the local structure of the graph around each node. 
A simple aggregate measure for this can be number of paths $p_i^l$ of a given length $l$ starting from each node $i$.
Since paths include repetitive movements, a better measure would be the number nodes $n_i^l$ within a distance $l$ from node $i$. 
Using this walk-based approach, we can label each node by the sequence $n_i =(n_i^1,...,n^{l_{\max}}_i) $.  
$n_i^1$ is the degree of node $i$ and in general we have 
\begin{equation}
    n_i^l = \theta(A^l) \mathbf{1} \label{eq:nil}
\end{equation}
using the Heaviside step function $\theta(x) = \{1, \mbox{ if} x>0; 0,\mbox{else}\} $ 

\subsection{Effect of Graph Diameter on Model Architecture}
The prominent feature of network diffusion is that it is Markovian and is only transmitted to first neighbors of each node, as in message-passing \nd{Review Neural Message Passing}, meaning $g_m(A)_{ij} \propto \theta(A_{ij})$. 
This puts a fundamental restriction on how diffusion spreads over the graph and how a GCN could find P0. 











Theoretical bounds on GCN-based architectures: 
\begin{itemize}
    \item Relation of depth with graph diameter: Can all nodes be reached? 
    \item Relation of depth with range of diffusion (as a function of $R_0$): How far can it have spread and is it causally possible to predict with $d$ layer GCN?
    \item Define node equivalence based of $R_0$: only nodes within a certain range can be equivalent. 
\end{itemize}



As the diffusion dynamics is Markovian,  the joint distribution can be factorized as   $P(\V{x}^{t+1}| \V{x}^t)$ governs the evolution of node states $\V{x}$. The following theorem guarantees the estimator using GNNs. 

\begin{theorem}
A graph neural network in the form of  can accurately estimate patient zero  with probability $\delta$, if the network..
\label{eqn:estimation}
\end{theorem}

% Denote a $N$- node graph as $G=(V, E)$, where $|V|=N$. The concatenation of node states at time step $t$ is denoted as $\V{x}^t \in \real^N$, every node $\V{x}_i$ can take three state: S(susceptible), I (infectious), R(recovery). The joint state space for $\V{x}$ is thus $3^N$.  
%  and the state transition matrix of the Markov chain is $P \in \real^{N\times N}$. We have the dynamics of the diffusion process as:
% \[\V{x}^{t+1} =  P\V{x}^{t}\]
% The graph structure imposes assumptions on $P$, meaning:
% \[P_{ij} = \begin{cases} 0 & A_{ij} =0\\
% p_{ij}>0 & \text{otherwise} \end{cases}\]
% here $A$ is the adjacency of the graph. 





\section{Backup 05-27-2020}


% \nd{Stochastic point process mean field here. }
We now present our theoretical analysis for the conditions to identify patient zero (P0). 
In simulations and real data we are not dealing with continuous probabilities, but rather point-processes, which are stochastic samplings of the probabilities. 
Solving the full stochastic model is difficult, so
we resort to the mean-field approximation and work with the transition probabilities instead. 
%
% Assume that we have graph $G(V,E)$ with $N = |V|$ vertices labeled by indices $i \in \{1,\cdots, N\} $ and edge set $E$ captured by the adjacency matrix entries $A_{ij}$ which are nonzero if $ i$ is connected to $j$. 
% We will mostly focus of undirected (i.e. $A_{ij} = A_{ji}$), unweighted graphs, though our results do not depend on this assumption. 
The epidemic spreading models described above are a special case of a general Reaction-diffusion (RD) process occurring on graphs \cite{colizza2007reaction}. 
The main characteristics of these processes is that they involve a message-passing step (e.g. an infection signal coming from neighbors of a node). 
The SIR and SEIR models are also Markovian and 
% Consider a Markovian network (graph) diffusion process where 
the probability $P(x_i^t= \mu)$ of node $i$ being in state $\mu\in \{S,I,...,R\} $ at time $t$ only depends on the probabilities at $t-1$. 
Denoting $p_{i}^\mu(t) \equiv P(x_i^t= \mu) $ again, a Markovian reaction-diffusion dynamics can be written as 
\begin{align}
    p_i^\mu(t+1) &= \sigma \pq{ \sum_{j} F\Big( \mathcal{A}_{ij} \cdot h(p_j)^\mu \Big) } %\cr 
    \label{eq:gen_diffusion}
\end{align}
% each node $i$ can be in a number of states $\mu $ (e.g. $S,I,R$) at time $t$ 
where $\mathcal{A}$ are a set of propagation rules for the message, 
% Since node $i$ can only be directly affected by state of node $j$ if there is a connection between them, i.e. if $A_{ij} \ne 0$, we have  
which are only nonzero where $A$ is nonzero, and $h(p_i)$ can mix the states $\mu$ but do not change the node index $i$.  
These functions can be expressed as 
\begin{align}
    \mathcal{A}_{ij}^{a} &= \theta(A_{ij}) f(A)_{ij} &
    h_a(p_i)^\mu = \sigma\pq{\sum_\nu W^\mu_{a,\nu} p_i^\nu + b^\mu}
    \label{eq:gh_RD}
\end{align}
where $\theta(\cdot)$ is the step function and $\sigma(\cdot)$ a nonlinear function.
% Dynamics of the form \eqref{eq:gen_diffusion} are a type of nonlinear Reaction-diffusion (RD) dynamics \nd{citation} 
% defined on graphs and have been used to describe epidemic spreading \cite{colizza2007reaction}. 
% For example, simple diffusion on a graph, we have two states $S,I$ and diffusion is changing the $S\to I$ state. 
The agent-based model \eqref{eq:p_i-expansion0} can be written in form of \eqref{eq:gen_diffusion} using $\sigma (x) = 1- \exp(x)$, $F(x) = \log(1- \beta x)$, and two set of functions $\mathcal{A}^1 = A$, $ \mathcal{A}^2 = \mathbf{I}$ and $h_1(p_i)^\mu =\delta_{\mu,I} p^I_i$,  $h_2(p_i)^\mu= \delta_{\mu,S} p^S_i,$. 
Similarly, the original SIR model can be derived using $\sigma(x) = x$, $F(x) = \beta x$ and the same $\mathcal{A}^a, h_a$ (Supp.  \ref{ap:SIR-RD}).

\out{
\paragraph{Point-processes} 
We will be focusing on point-processes (e.g. random walk), instead of continuous diffusion, meaning that the diffusion also involves a stochastic sampling where out of the nodes with $p_i^I(t) >0 $ some will go into $x_i^t = I$ state and some won't. 
This can be encoded in \eqref{eq:gen_diffusion} by adding a sampling step, converting $p_i^\mu$ to discrete states $\tilde{p}_i^\mu =\mathcal{F}(p_i)^\mu $ which decides the state $x_i^t$ by taking into account all $p_i^\nu$ for being in states $\nu = S,I,...$. 
Solving the full stochastic Markov chain model is difficult. 
We resort to the mean-field approximation and work with the transition probabilities instead. 
% \nd{Markov chain complex; to make it simpler we work with mean-field approach i.e. probabilities. }
}

\paragraph{Relation to Graph Neural Networks}
% In conclusion, the epidemic spreading models on graphs all fall under the umbrella of the 
The reaction-diffusion equations. \eqref{eq:gen_diffusion} and \eqref{eq:gh_RD} resemble the ansatz for general message-passing neural networks (MPNN) \cite{gilmer2017neural}.
% \begin{proposition}
    % A Reaction-diffusion system on a graph can be approximated using MPNN \cite{gilmer2017neural}, which in turn may be approximated using graph convolutional networks (GCN) \cite{kipf2016semi} with multiple propagation rules, residual connections and nonlinear aggregation function. 
% \end{proposition}
We choose the simpler architecture of GCN instead and extend it to learn the backward RD dynamics. 
% \nd{Has someone shown something in relation to this? Would "How powerful are GNN?" or our paper help here?}
The action of a graph convolutional network (GCN) \cite{kipf2016semi}, taking node features $h_i^\mu$ for node $i$ and feature channel $\mu$ as input, is given by 
\begin{align}
    F(A;h)^\mu_i & = \sigma\pq{\sum_j \mathcal{A}_{ij} \pq{h_j^\nu W_\nu^\mu + b^\mu } } 
\end{align}
Where we have allowed a bias term $b^\mu$.
The original propagation rule (PR)  $\mathcal{A}$ in GCN is $D^{-1/2} A D^{-1/2}$ in GCN, but other rules have also been employed in the literature. 
We make some modifications to our GCN-based architecture to make it more general. 
The details are described in sec. \ref{sec:model}.
% We may use multiple GCN models with different PR $\mathcal{A}$.
% For small values $\beta$, \eqref{eq:p_i-expansion0} reduces to a sum $\beta \sum_j A_{ij}p_j^I p_i^S$, which, except for the factor of $p_i^S$, is in the form of a simple GCN.
% Using multiple GCN layers interlaced with node-wise fully-connected layers between each layer and residual connections, the network should be able to approximate most RD processes.  
% The GCN aggregation function is a simple sum over the PR index $j$ contracted with the node features. 
% However, general nonlinear aggregation as $f_a$ in \eqref{eq:gen_diff_F}, as well as nonlinear functions like $h_a$ in \eqref{eq:gh_RD} have also been used in the literature, such as neural message passing architectures  
% \cite{gilmer2017neural}. 
% Hence, RD dynamics has the same structure as neural message-passing and graph neural networks based on these architectures should be able to learn the forward RD dynamics.
% \qed 

\subsection{Learning the Backward Dynamics}
\ry{make the connection for back-ward dynamics}
So far, we only talked about the forward RD dynamics and how it relates to MPNN, but finding patient zero requires learning the backward dynamics of \eqref{eq:gen_diffusion}. 
We wish to see if we can learn the backward dynamics  to find patient zero. 
Naively, one might expect that we need the inverse of the PR $\mathcal{A}$ to find P0. 
But we note that each node can only have been infected by its neighbors, so even in the backward dynamics the inference requires message passing over the same adjacency matrix and, hence, should again have the structure of \eqref{eq:gen_diffusion}. 
However, combinatorically, the problem should be very challenging, since in every MP step we need to include the new neighbors of each node to find who could have infected it, resulting in an exponentially growing set for P0 similar to the forward dynamics \eqref{eq:I(t)-epidemic}.
In general, if the infection had taken over most of the graph, with $|G_I|\sim O(N)$,  
we would have to deal with an exponentially growing set of candidate nodes as we moved backwards in time and finding P0 would be difficult. 
However, if the infection is still in early stages and $|G_I|\ll N$, we can argue that finding P0 should be tractable. 
To illustrate, consider random graphs, where the leading eigenvalue is roughly the average degree $\lambda_1 \approx \bk{d}$. 
With $R_0 = \beta \bk{d}/\gamma > 1$,
% we have an epidemic. 
% Since the spreading probability from each node $j$ to its neighbor $i$ is given by $\beta {A}_{ij} p_j$, if $ d_j > 1$, 
% the size of the infection grows over time, if the number of infected nodes is much smaller than the total number of nodes, meaning $|G_I|\ll N$. 
% In this situation, 
in early stages the number of infections grows exponentially as in \eqref{eq:I(t)-epidemic}. 
This produces an asymmetry between the forward and backward dynamics. 
In particular, when $R_0 \ll \bk{d_i}$ the number of nodes that can potentially have infected node $i$ is a small subset of its neighbors. 
Hence in random graphs when $|G_I| \ll N $, in every backward MP step infector nodes get at least $R_0$ messages, whereas receivers of infectious signals on average had only one infected neighbor.
Since $R_0>0$, this reinforcement of the MP signals on earlier infectors will shrink set of P0 candidates exponentially, making it tractable to make a prediction. 
Note that, after contagion, where $|G_I|\sim O(N)$ or if the the size of P0$\sim O(N)$, this asymmetry between forward and backward dynamics disappears and it should be difficult to find P0. 
In particular, if the diameter $G_I$ becomes the diameter of $G$, most likely we have $|G_I|\sim O(N)$. 
From \eqref{eq:I(t)-epidemic}, this can happen when $t_{\max{}}(\beta \lambda_1 - \gamma) \sim 1$. 
We expect the inference problem to see a sharp drop in accuracy around $t_{\max{}}$
\nd{Can we test this? Do we see the oppsite? }

% \nd{Derive the duality under $S \leftrightarrow I$ in the SI model. Relate that to SIR. Talk about entropy conditions. }

\ry{this says nothing about the learnability of the backward dynamics} 

\ry{I don't understand what is the theoretical take-away here}

\subsection{Detection Probability}
We analyze the probability of accurately recover the diffusion source given  the diffusion dynamics. 
The technical difficulty of the analysis stems from the (1) the presence of cycles in graphs (higher-order transmission) (2) the recovery state introduces additional uncertainty to the diffusion process (3) the exact time step of the snapshot is unknown.
%
Existing theoretical results mostly focus on the SI dynamics %without considering the removed state. 
% For the SI model 
(i.e. SIR with $\gamma=0$, meaning no recovery), with concrete results for trees using ``rumor centrality'' \cite{shah2011rumors}. 
Rumor centrality measures the closeness centrality of infected nodes to the last nodes being infected and the most central node is shown to be a maximum likelihood estimator for P0 on trees. 
Closeness centrality ranks the node by $\sum_j 1/d_{ij} $ where $d_{ij}$ is the graph distance between $i,j$, the intuition being that P0 should have a balanced distance from the boundary of the spreading. 
% For example, \cite{shah2011rumors} defines \textit{rumor centrality} to measure the probability of each node being the diffusion source. 
Intuitively, as the transmission is random, the infection sequences includes all possible permutations of the nodes, constrained by the topological order. Specifically, denote a  tree  of $N$ nodes with root $u$ as $T_N(u)$, the  rumor centrality is defined as
\begin{equation}
    R(N,u)= N! \frac{1}{\prod_{v\in {T}_N(u)} |T_N(v)|}
\end{equation}

The following theorem guarantees the success probability of identifying patient zero for a regular tree with degree $d$:
\begin{theorem}
Let $T_n(n)$ be a diffusion on a d-regular tree with degree $d\geq 3$, for any $\eta \in (0,1)$ and $k \geq 3$, 
\[\lim\sup_{n\rightarrow \infty} \mathbb{P}(M = \mathcal{A}^\star  ) \geq  C_1 \eta^{\frac{d-1}{d-2}} + C_2 k^{\frac{2d-3}{d-2}}(1-\eta)^{k-1+\frac{1}{d-2}}\]
with $M$ being the estimator using rumor centrality.
\end{theorem}

\ry{Analyze using Galton–Watson process/Branching Process}
% https://www.cs.cornell.edu/home/kleinber/networks-book/networks-book-ch21.pdf
In a $d$-regular tree, each $x_i$ affects $d$ neighbours with probability $\beta$. Let us focus on a quantity called \textit{basic reproductive number}, $R$, which the expected number of new cases infected by a single individual. Clearly for trees, if $Rd > 1$, the disease will continue to be contagious with probability larger than zero. There will be at least one node in $\V{x}^t$ that is infected and we can easily identify patient zero. If $Rd < 1$, then with probability $1$, the disease with die out. The probability of identifying patient zero after the disease dies out is zero. 




% \nd{
% 1) For binary graphs (degrees $d=3$) they predict a detection probability of $1/4$. Can you check if for $\gamma \to0$ or $\gamma \ll \beta $ GCN reaches this limit for high $t$?

% 2) How efficient is the rumor centrality compared to DMP and GCN? How does it scale with size of network?  
% }


% Given a dataset of  graph snapshots $\{\V{x}^t\}$ from an SIR dynamics, we wish the obtain the estimator for the problem in \eqref{eqn:patient_zero}. 
% The general loopy graph is difficult to analyze, we limit our analysis to irregular trees. The following result states the existence of an estimator for finding patient zero:
% \begin{theorem}[Existence\cite{bubeck2017finding}]
% There exist constants $c$, $c'>0$ such that the following holds true in the ER graph. Any root-finding algorithm must satisfy $K(\epsilon) \geq \exp(\sqrt{c\log(1/\epsilon})$.
% Furthermore, there exists a polynomial time root-finding algorithm with $K(\epsilon) \leq  \exp( c'\frac{\log(1/\epsilon)}{\log \log(1/\epsilon)})$. Here $K(\epsilon)$ is output top $K$ nodes with accuracy $\epsilon$ to find patient zero.
% \end{theorem}

\subsection{Difficulty of finding Patient Zero}
The task of finding P0 % requires learning the backward dynamics. 
% This task 
is compounded by the stochasticity of the infection spreading, resulting in different outcomes from the same initial conditions. 
We examine the possibility of establishing bounds on identifiability of P0 using a GCN-based model in in SIR-like dynamics on graphs. 
The main factors which affecting the ability to predict P0 are: (1) Ambiguity of patient zero; (2) Spreading radius of the infection relative to the diameter of the graph; (3) The parameters and type of the underlying epidemic model. 
% \begin{enumerate}
%     \item Ambiguity of patient zero,
%     \item Diameter of the graph, 
%     \item Spreading radius of the infection. 
%     \item The parameters and type of the underlying epidemic spreading model. \cs{Should we also mention dynamics of the underlying spread governed by $\beta$, $\gamma$}?
% \end{enumerate}
The ambiguity of P0 is due to some nodes being indistinguishable from each other, such as leaf nodes in a tree. 
The diameter, which is the maximum shortest distance between any pair of nodes, will affect how deep our GCN-based model needs to be in order to reach all potential P0. 
The spreading radius depends on the time passed since P0 as well as the parameters of the dynamics.
Combined with its upper boud, the graph diameter, the spreading radius will set a lower bound on the depth of the GCN model. 
Below, we explain how each of these factors plays a role and try to estimate their effect on identifying P0. 


% \subsection{Identifiability of Patient Zero}
\subsection{Ambiguity of Patient Zero}
\begin{wrapfigure}{r}{0.6\textwidth}
% \includegraphics[width=.5\linewidth]{figs/hash-infected-subgraph138-BA-5-k_max200.pdf}
\includegraphics[width=.49\linewidth]{figs/hash-infected-subgraph100-RGG-200-k_max5.pdf}
\includegraphics[width=.49\linewidth]{figs/hash-infected-subgraph115-BA-200-k_max5.pdf}
\caption{Equivalence classes of the quick hashing method inspired by the Weisfeiler-Lehman algorithm. 
Grey nodes are outside of the infected subgraph $G_I$. 
The colors indicate the equivalence classes. On the tree (right) $G_I$ has 115 nodes, but only $38$ distinct equivalence groups.
The Random Geometric Graph (left), however, with 100 infected nodes has 84 distinct groups. 
}
\label{fig:Ambiguity}
\vspace{-3mm}
\end{wrapfigure}
%
Compared to a random walk, epidemic spreading is more identifiable, as visited sites will change from the S state to a different state. 
\nd{ambiguity rooted in GI} 
% For the SI model (i.e. SIR with $\gamma=0$, meaning no recovery) concrete results have been for trees using ``rumor centrality'' \cite{shah2011rumors}. 
% Rumor centrality measures the closeness centrality of infected nodes to the last nodes being infected and the most central node is shown to be a maximum likelihood estimator for P0 on trees. 
% Closeness centrality ranks the node by $\sum_j 1/d_{ij} $ where $d_{ij}$ is the graph distance between $i,j$, the intuition being that P0 should have a balanced distance from the boundary of the spreading.
% For instance, in SI over a grid, the infection will look roughly circular after a long time and P0 is at the center of the circle. 
However, it may happen that the problem of finding P0 is unidentifiable 
when some nodes in the graph are identical. 
\ry{separate the analyze of trees and general graphs}
For instance, in a tree, if P0 is predicted to be a leaf, all leaves sharing the same parent are equally likely to be P0 \ry{this only happens if we have multiple patient zeros} \nd{no, even for a single P0, it's ambiguous.}. 
If some nodes are truly indistinguishable, 
%then an algorithm which predicts any of them as P0 is giving the right answer. 
our measure of accuracy should check P0 modulo an equivalence relations between nodes, i.e. automorphisms of the graph. 
% In such cases, we need to assess the accuracy of our prediction by grouping equivalent nodes together. 
% This equivalence is related to ``graph canonication'' and the graph isomorphism problem. 
We want to find nodes in the infected subgraph ${G}_I\subset {G}$ which can be mapped to each other via an element of the automorphism group $Q = \mathrm{Aut}({G}_I) \subset {G}$. \ry{this should come first}
% Consider a random walk on a star-shaped graph, which has one root node $v_0$ and $N-1$ leaf nodes $v_i$ and all edges are undirected, connecting only $v_0$ to $v_i$. 
% Let $x^t = (x_0^t,...x_{N-1}^t)$ represent the state of the walk on the graph at time $t$. 
% $x_i^t=1$ if the walker is at node $i$ at time $t$ and zero otherwise. 
% The probability of a state $x^t$ is given by 
% \begin{equation}
%     P(x_i^t=1|x_j^{t-1}) = \delta_{j0}(1-\delta_{i0}) + (1-\delta_{j0})\delta_{i0} 
% \end{equation}
% where the Kronecker delta $\delta_{ij}$ is $1$ if $i=j$ and zero otherwise. 
% Clearly, if at $ t=2$ the walker is not at the root node, it could have been in any of the leaf nodes at $t=0$. 
% Suppose we try to predict the $t=0$ position of the walker using machine learning. 
% In a naive approach, we would use the $t=2$ as input and ask the algorithm to return the precise index of the node at $t=0$. 
% This not only results in a performance equal to a random prediction (except never picking the root node), but may also lead to the model fitting the sampling noise. 
%
% The ambiguity described above is due to the fact that many nodes are equivalent to each other under certain dynamical processes on the graph.
% In the star graph above, any of the $(N-1)!$ shuffling of the leaf nodes looks exactly the same to the random walk. 
% These shuffling all result in graphs isomorphic to the original $G$ and constitute the automorphism group $\mathrm{Aut}(G)$. 
% In general, the set of nodes that are equivalent for a dynamical process can be mapped to each other using a subgroup $Q\subset  \mathrm{Aut}(G)$. 
Finding $\mathrm{Aut}(G_I)$ is relate to the Graph Isomorphism (GI) problem, which is a problem in NP, but not known whether or not it is NP-complete \cite{mckay1981practical}.
% To measure accuracy of finding P0, we need to group equivalent nodes under $\mathrm{Aut}(G_I)$. 
There exist many algorithms for GI \cite{MCKAY201494}, all of which are at least exponential in $N$. 
% Our goal of finding equivalent nodes under the action of $\mathrm{Aut}(G)$, is related to finding the graph invariant known as the canonical form, which in general can be as hard as GI.
We choose to use a simpler heuristic inspired by the Weisfeiler-Lehman (WS) graph kernel \cite{weisfeiler1968reduction, shervashidze2011weisfeiler}. 
The idea is to label the nodes by a sequence of numbers encoding the local structure of the graph around each node. 
A simple aggregate measure for this is % number of paths $p_i^l$ of a given length $l$ starting from each node $i$.
% Since paths include repetitive movements, a better measure would be 
the number nodes $n_i^{(l)}$ within a distance $l$ from node $i$. 
% Using this walk-based approach, 
Hence, we can label each node by the sequence $n_i =(n_i^{(1)},...,n^{(l_{\max})}_i) $.  
$n_i^{(1)}$ is the degree of node $i$ and we have $n_i^{(l)} = \theta(A_I^l) \mathbf{1}$
% \begin{equation}
%     n_i^l = \theta(A^l) \mathbf{1} \label{eq:nil}
% \end{equation}
with $A_I^l$ being the $l$th power of the adjacency matrix of the $G_I$ and $\theta(\cdot)$ the step function. % $\theta(x) = \{1, \mbox{ if} x>0; 0,\mbox{else}\} $ 
Figure \ref{fig:Ambiguity} shows that on trees there are many equivalent nodes, even non-leaf nodes.
However, the structure of contact networks where diseases spread is much more localized. A good proxy for contact networks is a Random Geometric Graph (RGG). 
Left of Figure \ref{fig:Ambiguity} shows that on RGG, the level of node equivalence is far less, with most nodes being distinguishable. 
In general, we find non-tree graphs with sufficient randomness (e.g. RGG and random graphs), there are very few equivalent nodes in small graphs. 
Hence, we neglect we believe in realistic settings this ambiguity won't play a major role in detectability of P0.  
\nd{but on tree BA we should definitely group nodes.}

\subsection{Effect of Graph Diameter on Model Architecture}
% The prominent feature of network diffusion is that it is Markovian and is only transmitted to first neighbors of each node, as in message-passing \nd{Review Neural Message Passing}, meaning $g_m(A)_{ij} \propto \theta(A_{ij})$. 
% This puts a fundamental restriction on how diffusion spreads over the graph and how a GCN could find P0. 
From \eqref{eq:gen_diffusion}, the MP step states that the state of node $i$ at time $t$ is only affected directly by its first neighbors at time $t-1$.
By induction, this means that at $t-\tau$, all nodes at most $\tau$ steps away from $i$ can have affected its state, meaning  
\begin{equation}
    p_i(t)^\mu = F_\tau\pq {\{p_j^\nu(t-\tau) |\nu=S,\cdots,R ; A_{ij}^\tau\ne0 \} }
    \label{eq:p(t-tau)}
\end{equation}
The $j$ for which $A_{ij}^\tau \ne 0 $ are the nodes at most $\tau$ steps away from $i$. 
Assuming $G$ is connected, define the diameter of graph $\mathrm{Dia}(G)\equiv \min_l{\pq{A_{ij}^l\ne 0, \forall i,j }}$, i.e. the maximum shortest distance between any two nodes.
Clearly, when $\tau \geq \mathrm{Dia}(G)$, the state of any node will depend on all other nodes in the past and the infection will have spread to all nodes ($|G_I|= |G| = N$).
Now, note that \eqref{eq:p(t-tau)} is a general statement about MP and not just about epidemics. 
It states that after $\tau$ steps of MP only the states of nodes up to a distance $\tau$ away from any given node can be passed in the messages. 
This leads to the following observation
\begin{proposition}
If a reaction diffusion dynamics has been spreading for $\tau$ time steps in a graph with diameter $\mathrm{Dia}(G)$, we need  $l_{MP} >\min{\pq{\tau,\mathrm{Dia}(G)}}$ layers of message-passing to be able to identify all patient zeros.  
\end{proposition}
After $\tau$ steps, P0 and the last infected nodes $i$ can be a graph distance $\tau$ apart. 
If the MP-based method is trying to maximize the probability $p_{P0}$ for the correct nodes to be patient zero, in general it would require to incorporate information about most infected nodes, which includes last infected nodes $i$. 
From \eqref{eq:p(t-tau)}, when $l_{MP} < \tau < \mathrm{Dia}(G)$, with $l_{MP}$ MP steps it is impossible for $p_{P0}$ to become a function of a node $i$ which is a distance of more than $l_{MP}$ away. 
Hence we need at least $\tau$ MP steps, unless $\tau > \mathrm{Dia}(G)$, in which case we can go from any node to any other with $l_{MP} = \mathrm{Dia}(G)$ MP steps. 
\qed

This observation means that any GCN-based or MPNN architecture we use doesn't need to be much deeper than the diameter of the graph. 
Random graphs generally have very short diameters, around $\mathrm{Dia}(G) \sim \log N$, but geographic graphs, such as RGG have larger diameters roughly $\mathrm{Dia}(G)\sim  N^{1/d}$ where $d$ is the dimensions of the space. 
For example, if there are no long-distance travels, the contact network of people in a town or city is roughly an RGG in 2D. 
With these limits in mind, we design a GCN-based architecture to learn P0 on multiple graphs and for different $R_0$ values. 

% Theoretical bounds on GCN-based architectures: 
% \begin{itemize}
%     \item Relation of depth with graph diameter: Can all nodes be reached? 
%     \item Relation of depth with range of diffusion (as a function of $R_0$): How far can it have spread and is it causally possible to predict with $d$ layer GCN?
%     \item Define node equivalence based of $R_0$: only nodes within a certain range can be equivalent. 
% \end{itemize}

% As the diffusion dynamics is Markovian,  the joint distribution can be factorized as   $P(\V{x}^{t+1}| \V{x}^t)$ governs the evolution of node states $\V{x}$. The following theorem guarantees the estimator using GNNs. 

% \begin{theorem}
% A graph neural network in the form of  can accurately estimate patient zero  with probability $\delta$, if the network..
% \label{eqn:estimation}
% \end{theorem}

% Denote a $N$- node graph as $G=(V, E)$, where $|V|=N$. The concatenation of node states at time step $t$ is denoted as $\V{x}^t \in \real^N$, every node $\V{x}_i$ can take three state: S(susceptible), I (infectious), R(recovery). The joint state space for $\V{x}$ is thus $3^N$.  
%  and the state transition matrix of the Markov chain is $P \in \real^{N\times N}$. We have the dynamics of the diffusion process as:
% \[\V{x}^{t+1} =  P\V{x}^{t}\]
% The graph structure imposes assumptions on $P$, meaning:
% \[P_{ij} = \begin{cases} 0 & A_{ij} =0\\
% p_{ij}>0 & \text{otherwise} \end{cases}\]
% here $A$ is the adjacency of the graph. 




==> secs/todo.tex <==
Diffusion processes are the simplest types of linear dynamics over graphs. 
Assume we have a graph of $N$ nodes. 
Let the adjacency matrix entry $A_{ij}$ denote the weight of the link from node $i$ to $j$ and the diagonal degree matrix entries be $D_{ij} = \delta_{ij} \sum_{k=1}^N A_{ik}$. 
The simple, discrete time diffusion process is defined using the diffusion operator $\hat{A} \equiv D^{-1} A$ as
\begin{align}
X_{t+1} &= \lambda \hat{A} X_t \\
\delta X_{t+1} &= (\lambda \hat{A} -I) X_t \label{eq:diffusion}.
\end{align}
While inverting the first equation requires matrix inversion, the second one can be expanded as a Taylor series, if $|\lambda| < 1$
\begin{align}
X_{t} &= (\lambda D^{-1}A -I)^{-1} \delta X_{t+1} %\cr 
% & = \left(\sum_{m=0}^\infty {(\lambda \hat{A})^m\over m!} \left.\partial^m (x-1)^{-1}\right|_{x=0} \right)\cr
% & = \left(\sum_{m=0}^\infty {(\lambda \hat{A})^m\over m!} m! (-1)^m (-1)^{-m-1} \right)X_t\cr 
= -\sum_{m=0}^\infty (\lambda \hat{A})^m \delta X_{t+1} \label{eq:expand-diffusion}
\end{align}
This means that for small enough Frobenius norms $\|\lambda \hat{A}\|$ the inverse dynamics can be efficiently approximated by keeping a small number $n_0$  of terms
\begin{equation}
    X_{t} \approx -\sum_{m=0}^{n_0} (\lambda \hat{A})^m \delta X_{t+1} 
\end{equation}
This can be efficiently implemented using a Graph Convolutional Network (GCN) \cite{kipf2016semi} ({\color{red} ND: Is this essentially the same as your diffusion convolution paper, Rose? }). 
However, the data of the dynamics may be noisy. 
Given time series data of the process over the nodes,  we wish to know whether we can find the graph structure underlying the process and how robust this prediction is. 

Note that $F = \beta I/N$ is called the infection force. 
Introducing the network adjacency matrix $A$, the equations change such that infections can only spread over the links of the network. 
This changes the infection force, but does not affect the recovery, which is a per node effect, nor the number conservation.
The infection force will now depend on what fraction of the neighbors of a node are infected. 
First, we need to define $I_i$ as 1 if node $i$ is infected, and zero otherwise. 
Then, the Infection force on node $i$ must be changed to the fraction of neighbors of $i$ which are infected.
Denoting the degree of nodes as $k_i = \sum_j A_{ij}$ and the degree matrix as $D_{ij} = k_i \delta_{ij}$, the infection force becomes
\begin{equation}
    F_{ij} = \beta {1\over k_i} A_{ij} I_j = \beta (D^{-1}A)_{ij} I_j. \label{eq:Fij}
\end{equation}

Defining the ``diffusion operator'' as $\hat{A} = D^{-1} A$, 
the network version of the SIR equations then become
\begin{align}
    {dS_i \over dt} &= - \beta \sum_j \hat{A}_{ij}I_j S_i \label{eq:net-dS} \\
    {dR_i \over dt} &= \gamma I_i \label{eq:net-dR} \\
    {dI_i \over dt} &= - {dS_i\over dt} - {dR_i\over dt} \label{eq:net-conserve}
\end{align}

Given a set of time series for $S,I,R$, can we extract $A, \beta$, and $\gamma$? 
Can the same procedure also be used to find ``patient zero''? 


The first step is to define a machine learning architecture that encodes precisely these equations. 
We have three features per node ($SIR$). 
The first equation \eqref{eq:net-dS} is similar to a GCN with linear activation, but it also has a factor of $S_i$ and it is a recurrent equation. 


The last equation is a constraint equation and has no learnable parameters, so we should implement it as a constraint. 
For input variables such as $S,I,R$ such constraints can easily be added to the loss function using regularization terms, which are Lagrange multipliers times the square of the constraint. 
However, it becomes slightly non-trivial when the constraints involve the time derivatives. 


we need to know the parameters of the dynamics and also how to run it backwards. 
For diffusion, running it backward is trivial, as we could simply invert the diffusion matrix. 
However, in SIR the first equation is difficult to run backwards. 
If we divide $dS_i$ by $S_i$ we get another equation that can be easily inverted. Like
\begin{align}
    S_{t+1,i} - S_{t,i} &= -\beta (A \cdot I_t)_i S_{t,i}\cr
    S_{t+1} / S_t - 1 &= -\beta A\cdot I_t\cr
    -\beta^{-1} A^{-1} \cdot (S_{t+1} / S_t) &= I_t 
\end{align}
The complication here is that in backward dynamics we only have the data for step $t+1$ and want to predict step $t$. 


\paragraph{SAIR model}
We can also have a more complicated model that portrays a more realistic image of an epidemic outbreak. We can now divide the infected state $I$ into two parts - $I_A$ and $I_S$ such that $I_A$ is an asymptomatic individual (but is still infected and capable of infecting susceptible nodes) and $I_S$ is a symptomatic individual. We introduce $\alpha$ as the probability of being an asymptomatic individual, we assume that an infected individual has the same infectivity. We define $\lambda$ as the probability that an asymptomatic individual will recover at $t$. Let $Q(i, t)$ be the query operator for node $i$ at time $t$ and therefore $Q(i, t) \in \{S, I_A, I_S, R\}$. We will use the shorthand $q^i_t$ for the operator. Let $\xi_i$ define the fraction of neighbours infected (symptomatic or asymptomatic), that is $\xi_i = \sum_j A_{ij}[q^j_{t-1} = I]$. We can now define an agent based model as follows:
\begin{align}
    P(q^j_t = I_A | q^i_{t-1} = S) &= \alpha[1 - (1 - \beta)^{\xi_i}] \label{eq:sair_infection_prob} \\
    P(q^j_t = I_S | q^i_{t-1} = S) &= (1 - \alpha)[1 - (1 - \beta)^{\xi_i}] \label{eq:sair_infection_prob} \\
    P(q^j_t = R | q^i_{t-1} = I_S) &= \gamma \label{eq:symptomatic_recovery} \\
    P(q^j_t = R | q^i_{t-1} = I_A) &= \lambda \label{eq:asymptomatic_recovery}
\end{align}
